ICE: Interactive 3D Game Character Editing via Dialogue

ost recent popular Role-Playing Games (RPGs) allow players to create in-game characters with hundreds of adjustable parameters, including bone positions and various makeup options. Although text-driven auto-customization systems have been developed to simplify the complex process of adjusting these intricate character parameters, they are limited by their single-round generation and lack the capability for further editing and fine-tuning. In this paper, we propose an Interactive Character Editing framework (ICE) to achieve a multi-round dialogue-based refinement process. In a nutshell, our ICE offers a more user-friendly way to enable players to convey creative ideas iteratively while ensuring that created characters align with the expectations of players. Specifically, we propose an Instruction Parsing Module (IPM) that utilizes large language models (LLMs) to parse multi-round dialogues into clear editing instruction prompts in each round. To reliably and swiftly modify character control parameters at a fine-grained level, we propose a Semantic-guided Low-dimension Parameter Solver (SLPS) that edits character control parameters according to prompts in a zero-shot manner. Our SLPS first localizes the character control parameters related to the fine-grained modification, and then optimizes the corresponding parameters in a low-dimension space to avoid unrealistic results. Extensive experimental results demonstrate the effectiveness of our proposed ICE for in-game character creation and the superior editing performance of ICE.

==> resource/sub_blocks/tab-exp-frt2p.tex <==
% \begin{tabular}{@{}l|ll@{}}
% \toprule
% \textbf{Method} & \textbf{CLIP score} & \textbf{Running time} \\ \midrule
% DreamFace       &  0.2362    & \textgreater{}300s    \\
% TADA            &  0.2689             & 4.5h                 \\
% T2P             &  0.2480    & 359.47s               \\
% FR-T2P(ours)    &  \textbf{0.2699}   & \textbf{2s}           \\ \bottomrule
% \end{tabular}


\begin{tabular}{@{}l|llll@{}}
\toprule
                      & DreamFace                           & TADA   & T2P     & ICE(Ours)             \\ \midrule
CLIP score $\uparrow$           & 0.2362                              & 0.2689 & 0.2480  & \textbf{0.2699} \\
Response time $\downarrow$        & \textgreater{}300s & 4.5h   & 359.47s & \textbf{3.34s}     \\ \midrule
Text consistency $\uparrow$ & 1.553                               & 1.937  & 2.066   & \textbf{3.756}  \\
Quality $\uparrow$              & 1.777                               & 1.882  & 2.089   & \textbf{4.061}  \\
Preference $\uparrow$           & 2.5\%                               & 13.0\% & 7.4\%   & \textbf{77.1\%} \\ \bottomrule
\end{tabular}


% \begin{tabular}{@{}c|ccccc@{}}
% \toprule
% \multirow{2}{*}{Methods} & \multicolumn{2}{c}{Objective Evaluations}                                  & \multicolumn{3}{c}{Subjective Evaluations}               \\
%                          & CLIP score      & \multicolumn{1}{c|}{Running time}                        & Consistency with text & Quality        & Preference      \\ \cmidrule(l){2-6} 
% DreamFace                & 0.2362          & \multicolumn{1}{c|}{\textgreater{}300s} & 1.553                 & 1.777          & 2.5\%           \\
% TADA                     & 0.2689          & \multicolumn{1}{c|}{4.5h}                                & 1.937                 & 1.882          & 13.0\%          \\
% T2P                      & 0.2480          & \multicolumn{1}{c|}{359.47s}                             & 2.066                 & 2.089          & 7.4\%           \\
% ICE                      & \textbf{0.2699} & \multicolumn{1}{c|}{\textbf{3.34s}}                      & \textbf{3.756}        & \textbf{4.061} & \textbf{77.1\%} \\ \bottomrule
% \end{tabular}

==> resource/sub_blocks/tab-exp-llm.tex <==
% \begin{tabular}{@{}lp{3cm}p{3cm}p{6cm}p{5cm}@{}}
% \toprule
% \textbf{Round}         & \textbf{User Input}                                                                    & \textbf{Response}                                           & \textbf{Parsed Command}                                                                                                                    & \textbf{Memory State}                                                                                                                                                                               \\ \midrule
% \multicolumn{1}{l|}{1} & A girl with big eyes                                                                   & Done!                                                       & {[}\{'target': 'Big eyes', 'strength': 0.5\}{]}                                                                                            & \{'Big eyes': '0.5'\}                                                                                                                                                                               \\
% \multicolumn{1}{l|}{2} & Even bigger                                                                            & Okay, the eyes are even bigger                              & {[}\{'target': 'Big eyes', 'strength': 0.7\}{]}                                                                                            & \{'Big eyes': '0.7'\}                                                                                                                                                                               \\
% \multicolumn{1}{l|}{3} & Still too small                                                                        & How does it look now?                                       & {[}\{'target': 'Big eyes', 'strength': 0.9\}{]}                                                                                            & \{'Big eyes': '0.9'\}                                                                                                                                                                               \\
% \multicolumn{1}{l|}{4} & Max it out                                                                             & Okay, it's now at its maximum size                          & {[}\{'target': 'Big eyes', 'strength': 1.0\}{]}                                                                                            & \{'Big eyes': '1.0'\}                                                                                                                                                                               \\
% \multicolumn{1}{l|}{5} & Can it be bigger?                                                                      & Sorry, it's already at its maximum size                     & {[}{]}                                                                                                                                     & \{'Big eyes': '1.0'\}                                                                                                                                                                               \\ \midrule
% \multicolumn{1}{l|}{1} & Majestic Empress                                                                       & Okay, I've adjusted it to the look of the Majestic Empress. & {[}\{'target': 'Majestic Empress', 'strength': 0.5\}{]}                                                                                    & \{'Majestic Empress': '0.5'\}                                                                                                                                                                       \\
% \multicolumn{1}{l|}{2} & Make the nose slightly higher, the eyes smaller and more spirited, and the mouth wider & I've made the adjustments, what do you think?               & {[}\{'target': 'High nose', 'strength': 0.6\}, \{'target': 'Small eyes', 'strength': 0.4\}, \{'target': 'Wide mouth', 'strength': 0.6\}{]} & \begin{tabular}[c]{@{}l@{}}\{\\     'Majestic Empress': '0.5',\\     'High nose': '0.6',\\     'Small eyes': '0.4',\\     'Wide mouth': '0.6'\\ \}\end{tabular}                                     \\
% \multicolumn{1}{l|}{3} & Change the lip makeup to make her look more majestic                                   & Done.                                                       & {[}\{'target': 'More majestic lip makeup', 'strength': 0.5\}{]}                                                                            & \begin{tabular}[c]{@{}l@{}}\{\\    'Majestic Empress': '0.5',\\    'High nose': '0.6',\\    'Small eyes': '0.4',\\    'Wide mouth': '0.6',\\    'More majestic lip makeup': '0.5'\\ \}\end{tabular} \\
% \multicolumn{1}{l|}{4} & Lower the nose a bit                                                                   & Okay, I've lowered the nose.                                & {[}\{'target': 'High nose', 'strength': 0.4\}{]}                                                                                           & \begin{tabular}[c]{@{}l@{}}\{\\    'Majestic Empress': '0.5',\\    'High nose': '0.4',\\    'Small eyes': '0.4',\\    'Wide mouth': '0.6',\\    'More majestic lip makeup': '0.5'\\ \}\end{tabular} \\
% \multicolumn{1}{l|}{5} & The adjustments are good, it's what I wanted                                           & I'm glad you like it.                                       & {[}{]}                                                                                                                                     & \begin{tabular}[c]{@{}l@{}}\{\\    'Majestic Empress': '0.5',\\    'High nose': '0.4',\\    'Small eyes': '0.4',\\    'Wide mouth': '0.6',\\    'More majestic lip makeup': '0.5'\\ \}\end{tabular} \\ \bottomrule
% \end{tabular}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{tabular}{@{}lp{3.5cm}p{6cm}p{5cm}@{}}
% \toprule
% \textbf{Round}         & \textbf{User Input}                                                                    & \textbf{Parsed Command}                                                                                                                    & \textbf{Memory State}                                                                                                                                                                               \\ \midrule
% \multicolumn{1}{l|}{1} & A girl with big eyes                                                                   & {[}\{'target': 'Big eyes', 'strength': 0.5\}{]}                                                                                            & \{'Big eyes': '0.5'\}                                                                                                                                                                               \\
% \multicolumn{1}{l|}{2} & Even bigger                                                                            & {[}\{'target': 'Big eyes', 'strength': 0.7\}{]}                                                                                            & \{'Big eyes': '0.7'\}                                                                                                                                                                               \\
% \multicolumn{1}{l|}{3} & Still too small                                                                        & {[}\{'target': 'Big eyes', 'strength': 0.9\}{]}                                                                                            & \{'Big eyes': '0.9'\}                                                                                                                                                                               \\
% \multicolumn{1}{l|}{4} & Max it out                                                                             & {[}\{'target': 'Big eyes', 'strength': 1.0\}{]}                                                                                            & \{'Big eyes': '1.0'\}                                                                                                                                                                               \\
% \multicolumn{1}{l|}{5} & Can it be bigger?                                                                      & {[}{]}                                                                                                                                     & \{'Big eyes': '1.0'\}                                                                                                                                                                               \\ \midrule
% \multicolumn{1}{l|}{1} & Majestic Empress                                                                       & {[}\{'target': 'Majestic Empress', 'strength': 0.5\}{]}                                                                                    & \{'Majestic Empress': '0.5'\}                                                                                                                                                                       \\
% \multicolumn{1}{l|}{2} & Make the nose slightly higher, the eyes smaller and more spirited, and the mouth wider & {[}\{'target': 'High nose', 'strength': 0.6\}, \{'target': 'Small eyes', 'strength': 0.4\}, \{'target': 'Wide mouth', 'strength': 0.6\}{]} & \begin{tabular}[c]{@{}l@{}}\{\\     'Majestic Empress': '0.5',\\     'High nose': '0.6',\\     'Small eyes': '0.4',\\     'Wide mouth': '0.6'\\ \}\end{tabular}                                     \\
% \multicolumn{1}{l|}{3} & Change the lip makeup to make her look more majestic                                   & {[}\{'target': 'More majestic lip makeup', 'strength': 0.5\}{]}                                                                            & \begin{tabular}[c]{@{}l@{}}\{\\    'Majestic Empress': '0.5',\\    'High nose': '0.6',\\    'Small eyes': '0.4',\\    'Wide mouth': '0.6',\\    'More majestic lip makeup': '0.5'\\ \}\end{tabular} \\
% \multicolumn{1}{l|}{4} & Lower the nose a bit                                                                   & {[}\{'target': 'High nose', 'strength': 0.4\}{]}                                                                                           & \begin{tabular}[c]{@{}l@{}}\{\\    'Majestic Empress': '0.5',\\    'High nose': '0.4',\\    'Small eyes': '0.4',\\    'Wide mouth': '0.6',\\    'More majestic lip makeup': '0.5'\\ \}\end{tabular} \\
% \multicolumn{1}{l|}{5} & The adjustments are good, it's what I wanted                                           & {[}{]}                                                                                                                                     & \begin{tabular}[c]{@{}l@{}}\{\\    'Majestic Empress': '0.5',\\    'High nose': '0.4',\\    'Small eyes': '0.4',\\    'Wide mouth': '0.6',\\    'More majestic lip makeup': '0.5'\\ \}\end{tabular} \\ \bottomrule
% \end{tabular}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tabular}{@{}cp{8cm}p{8cm}@{}}
\toprule
\textbf{Round}                                 & \textbf{User Input}                                                                    & \textbf{Parsed Command}                                                                                                                                                                  \\ \midrule
\multicolumn{1}{l|}{1}                         & A girl with big eyes                                                                   & {[}\{'target': 'Big eyes', 'strength': 0.5\}{]}                                                                                                                                          \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}2} & Even bigger                                                                            & {[}\{'target': 'Big eyes', 'strength': 0.7\}{]}                                                                                                                                          \\
\multicolumn{1}{l|}{3}                         & Still too small                                                                        & {[}\{'target': 'Big eyes', 'strength': 0.9\}{]}                                                                                                                                          \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}4} & Max it out                                                                             & {[}\{'target': 'Big eyes', 'strength': 1.0\}{]}                                                                                                                                          \\
\multicolumn{1}{l|}{5}                         & Can it be bigger?                                                                      & {[}{]}                                                                                                                                                                                   \\ \midrule
\multicolumn{1}{l|}{1}                         & Majestic Empress                                                                       & {[}\{'target': 'Majestic Empress', 'strength': 0.5\}{]}                                                                                                                                  \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}2} & Make the nose slightly higher, the eyes smaller and more spirited, and the mouth wider & \begin{tabular}[c]{@{}l@{}}{[}\{'target': 'High nose', 'strength': 0.6\},\\  \{'target': 'Small eyes', 'strength': 0.4\}, \\ \{'target': 'Wide mouth', 'strength': 0.6\}{]}\end{tabular} \\
\multicolumn{1}{l|}{3}                         & Change the lip makeup to make her look more majestic                                   & {[}\{'target': 'More majestic lip makeup', 'strength': 0.5\}{]}                                                                                                                          \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}4} & Lower the nose a bit                                                                   & {[}\{'target': \textbf{'High nose'}, 'strength': 0.4\}{]}                                                                                                                                         \\
\multicolumn{1}{l|}{5}                         & The adjustments are good, it's what I wanted                                           & {[}{]}                                                                                                                                                                                   \\ \bottomrule
\end{tabular}

==> resource/sub_blocks/tab-exp-quan.tex <==
\begin{tabular}{c|cc|ccc}
\toprule
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{Objective Evaluations}            & \multicolumn{3}{c}{Subjective Evaluations}              \\ \cline{2-6} 
                         & CLIP score      & Running time                        & Consistency with text & Quality        & Preference      \\ \midrule
DreamFace                & 0.2362          & \textgreater{}300s & 1.553                 & 1.777          & 2.5\%           \\
TADA                     & 0.2689          & 4.5h                                & 1.937                 & 1.882          & 13.0\%          \\
T2P                      & 0.2480          & 359.47s                             & 2.066                 & 2.089          & 7.4\%           \\
ICE                      & \textbf{0.2699} & \textbf{5.70s + 3.34s}              & \textbf{3.756}        & \textbf{4.061} & \textbf{77.1\%} \\ \bottomrule
\end{tabular}

==> sec/0_abstract.tex <==
\begin{abstract}
% Auto-creation systems for in-game characters have become increasingly popular in recent years, enabling users to personalize their Role-Playing Games (RPGs) experience. 
% However, existing character auto-creation systems are often static and limited to image or text-based optimization. 
% To address these limitations, we propose an interactive character creation method that allows users to modify their characters through a multi-round dialogue. 
% Our approach leverages a ChatGPT-based framework with a memory mechanism that accurately interprets user commands in context, and a neural network that ensures controllable modifications to character parameters. 
% We also introduce an improved method for editing facial parameters based on text input, which is both fast and controllable.
% Experimental results indicate that our interactive approach can accurately edit game characters according to user commands and lavoid irrelevant changes. 
% Ablation experiments demonstrate the effectiveness of our design.

% In-game character auto-creation systems have evolved, shifting from static image or text-based optimization to more dynamic methods. Addressing the limitations of traditional single-step creation methods, we present ICE, an Interactive Character Editing framework that enables users to iteratively modify their characters through a multi-round dialogue. This approach is more natural and enables finer control, avoiding inaccuracies due to overly complex single-step instructions.
% The landscape of in-game character auto-creation systems has predominantly been static, hinging on image or text-driven generation. Challenging this status quo, we introduce ICE, an Interactive Character Editing framework, marking the first shift towards a dynamic and interactive approach. This framework enables users to customize their 3D game characters through a multi-round dialogue, a more natural process that facilitates finer control and avoids inaccuracies due to overly complex single-step instructions.
% % Our framework consists of an instruction parser module employing a memory-augmented Large Language Model (LLM) to accurately interpret complex user inputs.
% % Our edition relevance predictor determines relevant areas and dimensions for editing based on text instructions, ensuring precise control over character parameters. Furthermore, we introduce a Fast and Robust Text-to-Parameter (FR-T2P) translation method facilitating quick and reliable text-driven character editing at each step.
% Our framework consists of an instruction parsing module and a character editing module.
% In the former module, we incorporates a memory mechanism into large language models (LLM), utilizing the powerful reasoning and interacting ability of memory-augmented LLM (MA-LLM) to extract refined editing instructions during dialogues and generate responses.
% In the latter module, we propose an edition relevance predictor and a fast and robust text-to-parameter (FR-T2P) translation method to follow the instructions and apply fine-gained control over 3D game characters while avoiding irrelevant changes.
% It provides reliable results within an acceptable response time.
% Experimental results affirm the accuracy and robustness of our framework, demonstrating its effectiveness through ablation studies.

% The in-game 3D character auto-creation systems from image or text input have been well developed in recent years. 
% However, existing generation methods are in a single-round manner, incapable of further refinement by interactive instructions. 
% Challenging this status quo, we propose an Interactive Character Editing framework (ICE), marking the first shift towards a multi-round and interactive approach. 
% Our framework enables users to customize their 3D game characters through a multi-round dialogue, a more natural process that facilitates finer control and avoids inaccuracies due to overly complex single-step instructions.
% Specifically, our framework disentangles the interactive generation into instruction parsing and character editing. 
% In the instruction parsing stage, we take the power of large language models (LLMs) to maintain a facial attribute memory bank and provide editing instructions based on natural dialogues.
% % incorporate a memory mechanism into large language models (LLM), creating memory-augmented LLM (MA-LLM) to improve the capability of reasoning and interacting. It understands user editing intentions from natural dialogues rather than structured direct instructions.
% In the character editing stage, we propose a mask-guided latent parameter solver to generate and edit character parameters according to the editing instructions.
% In order to provide reliable results within an acceptable response time, it iteratively optimizes character parameters in the latent space.
% Besides, it predicts and operates parameter channels relevant to the editing instructions, enabling fine-grained editing without irrelevant changes.
% Experimental results affirm the accuracy and robustness of our framework, demonstrating its effectiveness through ablation studies.

% Customized 3D characters, controlled by parameters such as facial bone positions, have been engaging in modern games and applications.
% Recently, text-driven auto-creation systems for 3D game characters are well developed, eliminating the need for players to manage hundreds of character parameters.
% However, existing generation methods are in a single-round manner, 
% incapable of further editing the character and fine-grained modifying the results.
% A more intuitive process is to interactively refine the character step by step through a multi-round dialogue, instead of forcing players to give a single-step comprehensive description.
% This interactive process is even necessary, as current methods often generate unrealistic results or mismatch certain parts of the description.
% There are several challenges to achieve the goal: 1) Understand multi-round dialogues and generate clear instruction prompts; 2) Fine-grained modification of the character without unintended changes; 3) Reliable generation of results and swift reaction in each step.
% Challenging this status quo,  we propose an Interactive Character Editing framework (ICE), marking the first shift towards a multi-round and interactive approach.  
% Specifically, we first propose an Instruction Parser (LP) module that utilizes large language models (LLMs) to understand multi-round dialogues and generate clear editing instruction prompts.
% To reliably and swiftly modify character parameters at a fine-grained level, we propose a Semantic-guided Latent Parameter Solver (MLPS) to edit character parameters according to prompts in a zero-shot manner.
% It contains a network to predict a mask of parameter channels for fine-grained modification, and it optimizes character parameters in a latent space to avoid unrealistic results.
% Experimental results affirm the accuracy and robustness of our framework, demonstrating its effectiveness through ablation studies.

% Text-driven in-game 3D character auto-creation systems have significantly advanced the customization of 3D characters in modern games and applications. 
% These systems eliminate the need for players to directly manipulate intricate character parameters, such as facial bone positions and other defined features. 

Text-driven in-game 3D character auto-customization systems eliminate the complicated process of manipulating intricate character control parameters.
However, current methods are limited by their single-round generation, incapable of further editing and fine-grained modification.
In this paper, we propose an Interactive Character Editing framework (ICE) to achieve a multi-round dialogue-based refinement process. 
In a nutshell, our ICE offers a more user-friendly way to enable players to convey creative ideas iteratively while ensuring that created characters align with the expectations of players.
Specifically, we propose an Instruction Parsing Module (IPM) that utilizes large language models (LLMs) to parse multi-round dialogues into clear editing instruction prompts in each round.
To reliably and swiftly modify character control parameters at a fine-grained level, we propose a Semantic-guided Low-dimension Parameter Solver (SLPS) that edits character control parameters according to prompts in a zero-shot manner.
Our SLPS first localizes the character control parameters related to the fine-grained modification, and then optimizes the corresponding parameters in a low-dimension space to avoid unrealistic results.
Extensive experimental results demonstrate the effectiveness of our proposed ICE for in-game character creation and the superior editing performance of ICE.
Project page: \url{https://iceedit.github.io/}.


\end{abstract}
